Sublinear Time and Space Algorithms for Correlation Clustering via Sparse-Dense Decompositions

We present a new approach for solving (minimum disagreement) correlation clustering that results in sublinear algorithms with highly efficient time and space complexity for this problem. In particular, we obtain the following algorithms for $n$-vertex $(+/-)$-labeled graphs $G$: -- A sublinear-time algorithm that with high probability returns a constant approximation clustering of $G$ in $O(n\log^2{n})$ time assuming access to the adjacency list of the $(+)$-labeled edges of $G$ (this is almost quadratically faster than even reading the input once). Previously, no sublinear-time algorithm was known for this problem with any multiplicative approximation guarantee. -- A semi-streaming algorithm that with high probability returns a constant approximation clustering of $G$ in $O(n\log{n})$ space and a single pass over the edges of the graph $G$ (this memory is almost quadratically smaller than input size). Previously, no single-pass algorithm with $o(n^2)$ space was known for this problem with any approximation guarantee. The main ingredient of our approach is a novel connection to sparse-dense graph decompositions that are used extensively in the graph coloring literature. To our knowledge, this connection is the first application of these decompositions beyond graph coloring, and in particular for the correlation clustering problem, and can be of independent interest.

==> lower-bounds.tex <==
% !TeX root = main.tex 
%!TEX root = main.tex

\newcommand{\Amat}{\ensuremath{\boldsymbol{M}\xspace}}
\newcommand{\CCalg}{\ensuremath{\textsf{ALG}\xspace}}
\newcommand{\Indalg}{\ensuremath{\textsf{PROT}\xspace}}

\newcommand{\istar}{\ensuremath{i^{\star}\xspace}}
\newcommand{\jstar}{\ensuremath{j^{\star}\xspace}}

\newcommand{\concate}[4]{\ensuremath{\textnormal{\textsf{Concate}}(#1,#2,#3,#4)}\xspace}

\newcommand{\clusone}{\ensuremath{\textsf{Cluster-1}\xspace}}
\newcommand{\clustwo}{\ensuremath{\textsf{Cluster-2}\xspace}}



\section{A Memory Lower Bound for the Exact Correlation Clustering in a Single Pass}
\label{sec:lb}
Following the semi-streaming algorithm with an $O(1)$ approximation in \Cref{sec:alg}, a natural question to ask is whether it is possible to obtain the exact answer of correlation clustering with a semi-streaming memory. In this section, we answer this question negatively: we show that any streaming algorithm that obtains the exact optimal answer for correlation clustering requires $\Omega\paren{n^{2}}$ memory, even the instances are restricted to complete graphs. The theorem also implies that our algorithm is asymptotically optimal for correlation clustering on complete graphs under the semi-streaming setup.  

We present the formal theorem as follows.
\begin{theorem}
\label{thm:cc-lb}
There exists a family of complete signed graphs $G=(V,E)$, such that any streaming algorithm that outputs the optimal solution for correlation clustering on $G$ with probability at least $\frac{99}{100}$ requires a memory of $\Omega\paren{n^{2}}$ bits.
\end{theorem}

\paragraph{High-level overview of the analysis.} On the high level, a natural strategy to design a adversary that works against correlation clustering algorithms is to hide a few `key edges' that determines the exact clusters. In particular, an adversarial instance can be as follows. Consider a complete graph with two cliques $C_{1}$ and $C_{2}$ which both contain $c$ vertices and only positive edges inside. Furthermore, consider one additional special vertex $v$ that is connected to $n_{1}$ vertices in $C_{1}$ and $n_{2}$ vertices in $C_{2}$ with positive edges, and both $n_{1}$ and $n_{2}$ takes a \emph{large fraction} of $c$. All other edges (e.g. edges between $C_{1}$ and $C_{2}$) are negative edges. As such, if we let $n_{1}\in \{n_{2}-1,\, n_{2}+1\}$, i.e. the number of positive edges that connect $v$ to $C_{1}$ and $C_{2}$ differs by exactly \emph{one}, the optimal solution will put $v$ and $C_{1}$ (respectively $C_{2}$) in the same cluster, and $C_{2}$ (respectively $C_{1}$) in another. However, if the streaming algorithm is only given an $o\paren{n^{2}}$ memory, it is hard for it to identify the `key edge' that determines the clique $v$ should be clustered with. As such, the algorithm cannot output the exact clusters on the adversarial instance with high probability. 

\subsubsection*{The Formal Proof of \Cref{thm:cc-lb}}
We now formalize the above intuitions and prove \Cref{thm:cc-lb}. Note that to formally prove space lower bound for graph streaming algorithms, it is not enough to work only with \emph{edges} as the algorithm may store other statistics. As such, we prove the theorem by a reduction argument based on the Communication Complexity. To proceed, we need to first introduce the following communication problem. 
\begin{problem}[Matrix INDEX]
\label{prb:mat-ind}
Suppose there are two players, namely Alice and Bob. Suppose Alice is given a binary matrix $\Amat \in \{0,1\}^{N\times N}$, and Bob is given a pair of integers $(\istar,\, \jstar)\in [N]\times [N]$. The goal of the two players is to output $\Amat(\istar,\jstar)$.
\end{problem}
Obviously, to output anything better than random guess, there have to be some messages communicated between the two players. Under the regime of one-way communication, i.e. Bob cannot send any message and Alice can only send a message to Bob \emph{once}, it is well known that the Matrix INDEX is hard in terms of the communication complexity.

\begin{proposition}[Communication Complexity of Matrix INDEX]
\label{prop:cc-mat-ind}
Any one-way randomized protocol that outputs the correct answer of Matrix INDEX with probability at least $\frac{49}{50}$ requires $\Omega\paren{N^{2}}$ bits of communication.
\end{proposition}
\chen{do we need to prove this or is it so standard that we don't have to worry?}

Our plan for the reduction proof goes as follow. Suppose, for the purpose of contradiction, there exists a streaming algorithm $\CCalg$ that returns the optimal solution for correlation clustering with probability at least $\frac{99}{100}$ and uses a memory of $o\paren{n^{2}}$ bits. We will show that it implies a communication protocol $\Indalg$ with $o\paren{N^{2}}$ bits of communication that is able to output $\Amat(\istar,\jstar)$ in \Cref{prb:mat-ind} with probability at least $\frac{49}{50}$. This contradicts \Cref{prop:cc-mat-ind}, which means such an $\CCalg$ cannot exist.

We now formally give the protocol $\Indalg$ conditioning on the streaming algorithm $\CCalg$. To proceed, we first introduce a notation: for a collection of vertices $V$ (ordered arbitrarily), we use $V(i)$ to denote the $i$-th vertex. We also present the following helper function that is going to be used repeatedly in the the protocol. The helper function \textsf{Concate} takes the following inputs: a set of vertices, namely $Z$, a special index $i' \in [|Z|]$, and two connected components $\textsf{Comp}_{1}$ and $\textsf{Comp}_{2}$. The function partitions the vertices $Z$ into $X$ and $Y$, but leave out a special vertex $L(i')$. For every vertex $v\in X$, the helper function adds a positive edge to every $u \in \textsf{Comp}_{1}$ and a negative edge to every $z \in \textsf{Comp}_{2}$; conversely, for every vertex $v \in Y$, the helper function adds a positive edge to every $u \in \textsf{Comp}_{2}$ and a negative edge to every $z \in \textsf{Comp}_{1}$. The formal description is as follows.

\begin{tbox}
\paragraph{A helper function:} $\concate{Z}{i'}{\textsf{Comp}_{1}}{\textsf{Comp}_{2}}$:
\begin{enumerate}[label=$(\roman*)$]
\item For every vertex in $Z$ \emph{except} $Z\paren{i'}$, arbitrarily partition them as $Z\setminus \{Z\paren{i'}\} = X\cup Y$. If $|Z|$ is an odd number, let $|X|=|Y|$; otherwise, let $|X|=|Y|+1$.
\item For every vertex $v \in X$, add a positive edge to every $u \in \textsf{Comp}_{1}$ and a negative edge to every $z \in \textsf{Comp}_{2}$.
\item For every vertex $v \in Y$, add a positive edge to every $u \in \textsf{Comp}_{2}$ and a negative edge to every $z \in \textsf{Comp}_{1}$.
\end{enumerate}
\end{tbox}

We are now ready to present the protocol. For simplicity, we assume $N$ is an odd number.

\begin{tbox}
$\Indalg$: a communication protocol.

\smallskip

\paragraph{Inputs:}
\begin{itemize}
\item $\CCalg$: a streaming algorithm that uses a memory of $o\paren{n^2}$ bits and outputs the optimal correlation clustering for any signed complete graph with probability at least $\frac{99}{100}$.
\item A matrix $\Amat \in \{0,1\}^{N\times N}$ to Alice.
\item A pair of integers $(\istar,\, \jstar)\in [N]\times [N]$ to Bob.
\end{itemize}

\smallskip

\paragraph{The Construction:} Alice and Bob construct a graph $G=(V,\, E)$ as follows.
\begin{enumerate}[label=$(\roman*)$]
	\item Both Alice and Bob construct $V$ with $n=203\cdot N$ vertices. Group them in the following manner:
	\begin{enumerate}
	    \item Let $L$, $B$ and $R$ be three group of $N$ vertices. % For every $i \in [N]$, we use $L(i)$, $B(i)$ and $R(i)$ to denote the $i$-th vertex in $L$, $B$ and $R$, respectively.
	    \item Let $C_{1}$, $C_{2}$ be two groups of $100\cdot N$ vertices.
	\end{enumerate}
	\item \textbf{Alice}: add edges between $L$ and $B \cup R$ based on the value of $\Amat\paren{i,j}$:
	\begin{itemize}
	    \item If $\Amat(i,j)=0$, add a positive edge between $L_{i}$ and $B_{j}$ and a negative edge between $L_{i}$ and $R_{j}$.
	    \item If $\Amat(i,j)=1$, add a positive edge between $L_{i}$ and $R_{j}$ and a negative edge between $L_{i}$ and $B_{j}$.
	\end{itemize}
	\item \textbf{Bob}: add edges by the following procedure:
	\begin{enumerate}
	    \item \textbf{Part I: Edges between $C_{1}\cup C_{2}\cup R \cup B$}:
	    \begin{enumerate}
    	    \item \label{line:ini-step} Add positive edges between the vertices inside $C_{1}$ and $C_{2}$ (I.e. make two cliques of positive edges).
    	    \item For the vertex set $B$, add edges with $\concate{B}{\jstar}{C_{1}}{C_{2}}$.
    	    \item Similarly, for the vertex set $R$, add edges with $\concate{R}{\jstar}{C_{1}}{C_{2}}$.
    	    \item \label{line:last-step} For every pair of vertices $(u,v)$ that are connected to $C_{1}$ with positive edges, add a positive edge between $u$ and $v$. Apply the same rule to the pairs connected to $C_{2}$ with positive edges.
    	    \item  Add negative edges between all the pair of vertices in $B\cup R\cup C_{1}\cup C_{2}$ that are not specified for an edge in the previous steps (Line~\ref{line:ini-step} to \ref{line:last-step}).
	    \end{enumerate}
	    \item \textbf{Part II: Edges between $C_{1}\cup C_{2}$ and $L$:} \par
	    For the vertex set $L$, add edges with $\concate{L}{\istar}{C_{1}}{C_{2}}$.
	    \item \textbf{Part III: Handling $L(\istar)$, $B(\jstar)$ and $R(\jstar)$:} 
	    \begin{enumerate}
	        \item Add positive edges between $L(\istar)$ and vertices in both $C_{1}$ and $C_{2}$.
	        \item Add positive edges between $B(\jstar)$ and vertices in $C_{1}$ and the vertices connected to $C_{1}$ with positive edges; conversely, add negative edges between $R(\jstar)$ and vertices in $C_{2}$ and the vertices connected to $C_{2}$ with positive edges.
	        \item Add positive edges between $R(\jstar)$ and vertices in $C_{2}$ and the vertices connected to $C_{2}$ with positive edges; conversely, add negative edges between $B(\jstar)$ and vertices in $C_{1}$ and the vertices connected to $C_{1}$ with positive edges.
	    \end{enumerate}
	\end{enumerate}
\end{enumerate}

\smallskip

\paragraph{The Message and Output: }
\begin{enumerate}[label=$(\roman*)$]
	\item Alice runs $\CCalg$, and send the memory of the algorithm as the message to Bob.
	\item Bob runs $\CCalg$ based on Alice's message, and outputs as follows:
	\begin{enumerate}
	    \item \label{line:return-rule-A} $\Amat\paren{\istar, \jstar}=0$, if $L(\istar)$ is clustered with vertices of $C_{1}$.
	    \item \label{line:return-rule-B} $\Amat\paren{\istar, \jstar}=1$, otherwise.
	\end{enumerate}
\end{enumerate}

\end{tbox}

The graph construction in $\Indalg$ seems complicated. Nevertheless, there is a straightforward picture for the final graph $G$ created by Alice and Bob. Note that on Bob's side, the construction essentially creates two cliques (of positive edges). The first clique contains all the vertices in $C_{1}$, half of the vertices of both $B$ and $R$ (except $B\paren{\jstar}$ and $R\paren{\jstar}$), and $B\paren{\jstar}$; Similarly, the second clique contains all the vertices in $C_{2}$, (the other) half of the vertices of both $B$ and $R$ (except $B\paren{\jstar}$ and $R\paren{\jstar}$), and $R\paren{\jstar}$. Furthermore, Bob evenly distributes vertices in $L$ (except $L\paren{\istar}$) to the above cliques, and the connections of positive edges are almost complete. As such, all the positive and negative edges assigned by Alice no longer affects the clustering outcome, \emph{except} $L(\istar)$. For this special vertex, Bob assign positive connections evenly to the first and the second clique. Hence, the optimal answer become dependent \emph{entirely} on whether $L(\istar)$ connects to $B\paren{\jstar}$ or $R\paren{\jstar}$. An illustration of the graph $G$ can be shown as \chen{We need another figure here}.

We now formally show that $\Indalg$ can solve \Cref{prb:mat-ind} with probability at least $\frac{99}{100}$ with $o\paren{N^{2}}$ bits of communication. The bits of communication is trivial since the memory of the streaming algorithm is $o\paren{n^{2}} = o\paren{N^{2}} $ bits, and Alice only sends the memory as the message to Bob. Therefore, we only need to show the correctness of $\Indalg$ with the following lemma.
\begin{lemma}
\label{lem:correct-Ind}
Conditioning on the correctness of $\CCalg$, $\Indalg$ always return the correct answer of $\Amat\paren{\istar, \jstar}$.
\end{lemma}
\begin{proof}
To prove the lemma, it suffices to show that $\Amat\paren{\istar, \jstar}=0$ \emph{if and only if} $L(\istar)$ is in the same clusters of $C_{1}$ in the optimal clustering $\OPT$. The `if' direction is trivial by the correctness of $\CCalg$ and the returning rule of Line~\ref{line:return-rule-A}. Therefore, we devote the effort to prove the `only if' direction.

Consider the case when $\Amat\paren{\istar, \jstar}=0$, we claim that the optimal clustering $\OPT$ has two clusters as follows:
\begin{itemize}
\item \clusone: All the vertices of $C_{1}$; vertices that are connected to $C_{1}$ with positive edges in $L$, $B$, and $R$ (except $L(\istar)$, $R(\jstar)$, and $B(\jstar)$); $B(\jstar)$; $L(\istar)$.
\item \clustwo: All the vertices of $C_{2}$; vertices that are connected to $C_{2}$ with positive edges in $L$, $B$, and $R$ (except $L(\istar)$, $R(\jstar)$, and $B(\jstar)$); $R(\jstar)$.
\end{itemize}
We can prove the optimality of the above clustering by showing that any other clustering only leads to higher costs. To see this, we first show that $\clusone$ and $\clustwo$ are optimal for every vertex other than $L\paren{\istar}$. We prove this for $\clusone$ by showing that moving any subset of vertices in $\clusone\setminus \{L\paren{\istar}\}$ to some new cluster ($\clustwo$ or a new cluster) results in higher costs. The case of $\clustwo$ follows in the same manner.

% \begin{minipage}{\dimexpr\textwidth-3cm}
\noindent
\hspace{2em}%
\begin{minipage}{0.95\textwidth}

\smallskip

\paragraph{Part 1: Vertices in $C_{1}$.} Note that for every vertex $v \in C_{1}$, it has \emph{no} negative edge in $\clusone$. Therefore, moving any subset of vertices of $C_{1}$ to any other cluster does \emph{not} result in a lower cost. Hence, $\OPT$ must keep \emph{all} the vertices in $C_{1}$ inside $\clusone$.

\medskip

\paragraph{Part 2: Vertices in $B \cup R \cup L \setminus \{L(\istar), B(\jstar)\}$.} Conditioning on Part 1, moving any vertex as such outside $\clusone$ result in an extra cost of at least $100\cdot N$ (since at least $100\cdot N$ positive edges are going to be separated). On the other hand, each vertex in $B \cup R \cup L \setminus \{L(\istar), B(\jstar)\}$ has at most $N$ negative edges that are \emph{not} separated already by $\clusone$ and $\clustwo$ (only the negative edges between the vertices in $L$). Therefore, moving any subset of $B \cup R \cup L \setminus \{L(\istar), B(\jstar)\}$ outside $\clusone$ leads to only higher costs.

\medskip

\paragraph{Part 3: Vertex $B\paren{\jstar}$.} Similar to the vertices of Part 2, moving $B\paren{\jstar}$ to another clusters separates at least $100\cdot N$ positive edges (conditioning on Part 1), and the number of negative edges we can gain is at most $N$. Hence, $\OPT$ will always put $B\paren{\jstar}$ in $\clusone$.

\smallskip

\end{minipage}

We now handle the vertex $L\paren{\istar}$. Note that $L\paren{\istar}$ has at least $100\cdot N$ positive edges to both $\clusone$ and $\clustwo$. Therefore, making it a singleton cluster yields in a much higher cost. On the other hand, if one moves $L\paren{\istar}$ to $\clustwo$, we show that there is an extra cost of $2$. To see this, note that apart from $B\paren{\jstar}$ and $R\paren{\jstar}$, $L\paren{\istar}$ has equal number of positive and negative edges in $\clusone$ and $\clustwo$. To give more details, recall that we assume $N$ is an odd number, and apart from $\jstar$, whenever $B(j)$ with a positive (resp. negative) edge to $L\paren{\istar}$ is assigned to $\clusone$, $R(j)$ with a negative (resp. positive) edge is also assigned to $\clusone$. Finally, by the construction rule, when $\Amat\{\istar, \jstar\}=0$, a positive edge is applied to $B\paren{\jstar}$ and a negative one to $R\paren{\jstar}$. Therefore, if one switches $L\paren{\istar}$ to $\clustwo$, the cluster pays for an extra pair of positive and negative edges. Hence, the optimal cluster $\OPT$ will always keep $L\paren{\istar}$ in $\clusone$.

Now we have shown $\OPT$ follows the scheme of $\clusone$ and $\clustwo$, which means $L\paren{\istar}$ is in the same cluster of $C_{1}$, as desired. \Qed{\Cref{lem:correct-Ind}}

\end{proof}

\begin{remark}
By the proof of \Cref{lem:correct-Ind}, it is straightforward to see that if $\Amat\{\istar, \jstar\}=1$, $L\paren{\istar}$ will stay in the same cluster of $C_{2}$ under the optimal clustering $\OPT$. Hence, Line~\ref{line:return-rule-B} can be modified to a condition as such. In this way, the protocol also gains some abilities to report failure if the clusters does not fall into the two cases. As a proof for the lower bound, such a modification does not improve anything on its own; yet it is interesting to point out and it might be of arithmetic values elsewhere.
\end{remark}

We can now wrap up the proof of \Cref{thm:cc-lb}. By \Cref{lem:correct-Ind}, the success probability of $\Indalg$ is at least
\begin{align*}
\Pr\paren{\text{\Indalg  is correct}} &\geq \Pr\paren{\text{$\CCalg$  is correct}}\cdot \Pr\paren{\text{\Indalg  is correct}\mid\text{$\CCalg$ is correct}} \tag{by ignoring the success probability when $\CCalg$ is incorrect}\\
&\geq \frac{99}{100}\cdot 1 \tag{by the assumption of $\CCalg$ and \Cref{lem:correct-Ind}}\\
&> \frac{49}{50}.
\end{align*}
And the communication complexity is $o(n^{2})=o(N^{2})$ bits since $n=203\cdot N$. This contradicts \Cref{prop:cc-mat-ind}, which implies that such an algorithm $\CCalg$ cannot exist. \Qed{\Cref{thm:cc-lb}}










